Amodal Cityscapes: A New Dataset, its Generation, and an Amodal Semantic Segmentation Challenge Baseline

Amodal perception terms the ability of humans to imagine the entire shapes of occluded objects. This gives humans an advantage to keep track of everything that is going on, especially in crowded situations. Typical perception functions, however, lack amodal perception abilities and are therefore at a disadvantage in situations with occlusions. Complex urban driving scenarios often experience many different types of occlusions and, therefore, amodal perception for automated vehicles is an important task to investigate. In this paper, we consider the task of amodal semantic segmentation and propose a generic way to generate datasets to train amodal semantic segmentation methods. We use this approach to generate an amodal Cityscapes dataset. Moreover, we propose and evaluate a method as baseline on Amodal Cityscapes, showing its applicability for amodal semantic segmentation in automotive environment perception. We provide the means to re-generate this dataset on github.

==> classdistributionperson.tex <==
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\small}}
\definecolor{cityscapes}{RGB}{255,203,35}%247,125,0}
\definecolor{amcs}{RGB}{56,125,224}
% \definecolor{color0}{rgb}{0,0.39,0.39}
% \definecolor{color1}{rgb}{1,0.4,0.45}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows}
\usetikzlibrary{backgrounds}
\usetikzlibrary{shapes}
\usetikzlibrary{arrows.meta}
\pgfplotsset{scaled x ticks=false}
\pgfplotsset{scaled y ticks=false}
%\tikzstyle{arrowaxes} = [-{Straight Barb[angle'=60,scale=2]}, line width=0.45mm]

\begin{axis}[
grid=both,
tick align=outside,
tick pos=left,
title={},
axis lines = left,
axis line style=-angle 60,
width=0.5\textwidth,
height = 0.23\textwidth,
x grid style={white!69.0196078431373!black},
xlabel style={align=center},
xlabel={\small $\kappa =$ number of person \small pixels per image},
xmin=-31169.4494873047, xmax=654558.449975586,
xtick style={color=black},
xticklabels={0,,200000,,400000,,600000},
y grid style={white!69.0196078431373!black},
ylabel style={align=center},
ylabel={\small percentage of images with \\ \small  $\kappa$ person pixels},
ymin=0, ymax=5.4578326960496e-05,
ytick style={color=black},
ytick={0,0.00001,0.00002,0.00003,0.00004,0.00005,0.00006},
yticklabels={0,0.001,0.002,0.003,0.004,0.005,0.006},
]
\draw[draw=none,fill=cityscapes] (axis cs:0.00048828125,0) rectangle (axis cs:12467.779296875,5.19793590099962e-05);
\draw[draw=none,fill=cityscapes] (axis cs:12467.7802734375,0) rectangle (axis cs:24935.55859375,9.94833167774305e-06);
\draw[draw=none,fill=cityscapes] (axis cs:24935.55859375,0) rectangle (axis cs:37403.3359375,4.6371630964715e-06);
\draw[draw=none,fill=cityscapes] (axis cs:37403.33984375,0) rectangle (axis cs:49871.12109375,3.58571276288162e-06);
\draw[draw=none,fill=cityscapes] (axis cs:49871.1171875,0) rectangle (axis cs:62338.89453125,2.34554216623472e-06);
\draw[draw=none,fill=cityscapes] (axis cs:62338.8984375,0) rectangle (axis cs:74806.6796875,1.45585330222261e-06);
\draw[draw=none,fill=cityscapes] (axis cs:74806.6796875,0) rectangle (axis cs:87274.4609375,1.1592905925106e-06);
\draw[draw=none,fill=cityscapes] (axis cs:87274.4609375,0) rectangle (axis cs:99742.2421875,9.70568868148409e-07);
\draw[draw=none,fill=cityscapes] (axis cs:99742.2421875,0) rectangle (axis cs:112210.0234375,8.08807390123674e-07);
\draw[draw=none,fill=cityscapes] (axis cs:112210.015625,0) rectangle (axis cs:124677.7890625,4.85284738160949e-07);
\draw[draw=none,fill=cityscapes] (axis cs:124677.796875,0) rectangle (axis cs:137145.578125,5.39204926749116e-07);
\draw[draw=none,fill=cityscapes] (axis cs:137145.578125,0) rectangle (axis cs:149613.359375,4.04403695061837e-07);
\draw[draw=none,fill=cityscapes] (axis cs:149613.359375,0) rectangle (axis cs:162081.140625,2.96562709712014e-07);
\draw[draw=none,fill=cityscapes] (axis cs:162081.140625,0) rectangle (axis cs:174548.921875,1.34801231687279e-07);
\draw[draw=none,fill=cityscapes] (axis cs:174548.921875,0) rectangle (axis cs:187016.703125,1.61761478024735e-07);
\draw[draw=none,fill=cityscapes] (axis cs:187016.703125,0) rectangle (axis cs:199484.484375,2.15681970699646e-07);
\draw[draw=none,fill=cityscapes] (axis cs:199484.484375,0) rectangle (axis cs:211952.265625,1.61761478024735e-07);
\draw[draw=none,fill=cityscapes] (axis cs:211952.265625,0) rectangle (axis cs:224420.046875,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:224420.0625,0) rectangle (axis cs:236887.828125,5.39205602497862e-08);
\draw[draw=none,fill=cityscapes] (axis cs:236887.8125,0) rectangle (axis cs:249355.59375,1.07840985349823e-07);
\draw[draw=none,fill=cityscapes] (axis cs:249355.59375,0) rectangle (axis cs:261823.375,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:261823.359375,0) rectangle (axis cs:274291.125,5.39204926749116e-08);
\draw[draw=none,fill=cityscapes] (axis cs:274291.1875,0) rectangle (axis cs:286758.96875,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:286758.9375,0) rectangle (axis cs:299226.71875,5.39204926749116e-08);
\draw[draw=none,fill=cityscapes] (axis cs:299226.75,0) rectangle (axis cs:311694.53125,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:311694.5,0) rectangle (axis cs:324162.28125,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:324162.3125,0) rectangle (axis cs:336630.09375,0);
\draw[draw=none,fill=cityscapes] (axis cs:336630.0625,0) rectangle (axis cs:349097.84375,5.39204926749116e-08);
\draw[draw=none,fill=cityscapes] (axis cs:349097.875,0) rectangle (axis cs:361565.65625,0);
\draw[draw=none,fill=cityscapes] (axis cs:361565.625,0) rectangle (axis cs:374033.40625,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:374033.4375,0) rectangle (axis cs:386501.21875,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:386501.1875,0) rectangle (axis cs:398968.96875,0);
\draw[draw=none,fill=cityscapes] (axis cs:398969,0) rectangle (axis cs:411436.78125,5.39204926749116e-08);
\draw[draw=none,fill=cityscapes] (axis cs:411436.75,0) rectangle (axis cs:423904.53125,8.08807390123674e-08);
\draw[draw=none,fill=cityscapes] (axis cs:423904.5625,0) rectangle (axis cs:436372.34375,8.08807390123674e-08);
\draw[draw=none,fill=cityscapes] (axis cs:436372.3125,0) rectangle (axis cs:448840.09375,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:448840.125,0) rectangle (axis cs:461307.90625,0);
\draw[draw=none,fill=cityscapes] (axis cs:461307.875,0) rectangle (axis cs:473775.625,2.6960313912415e-08);
\draw[draw=none,fill=cityscapes] (axis cs:473775.625,0) rectangle (axis cs:486243.40625,0);
\draw[draw=none,fill=cityscapes] (axis cs:486243.4375,0) rectangle (axis cs:498711.21875,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:498711.1875,0) rectangle (axis cs:511178.96875,0);
\draw[draw=none,fill=cityscapes] (axis cs:511179,0) rectangle (axis cs:523646.78125,2.69602463374558e-08);
\draw[draw=none,fill=cityscapes] (axis cs:523646.71875,0) rectangle (axis cs:536114.5,0);
\draw[draw=none,fill=cityscapes] (axis cs:536114.5625,0) rectangle (axis cs:548582.3125,0);
\draw[draw=none,fill=cityscapes] (axis cs:548582.375,0) rectangle (axis cs:561050.1875,5.39203575256706e-08);
\draw[draw=none,fill=cityscapes] (axis cs:561050.125,0) rectangle (axis cs:573517.875,0);
\draw[draw=none,fill=cityscapes] (axis cs:573517.875,0) rectangle (axis cs:585985.6875,0);
\draw[draw=none,fill=cityscapes] (axis cs:585985.6875,0) rectangle (axis cs:598453.4375,0);
\draw[draw=none,fill=cityscapes] (axis cs:598453.5,0) rectangle (axis cs:610921.3125,0);
\draw[draw=none,fill=cityscapes] (axis cs:610921.25,0) rectangle (axis cs:623389,2.6960313912415e-08);
\end{axis}

%\draw[draw=none,fill=color0] (2.06,4) rectangle (2.56,4.5);
%\node[text width=16cm, align=center] (v1) at (4.53,4.25) {\LARGE predicted (Pred)};
\end{tikzpicture}

==> occlusionhistogram.tex <==
\usetikzlibrary{arrows}
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmajorgrids,
width=0.5\textwidth,
height = 0.3\textwidth,
xmin=-0.031, xmax=0.23,
xtick style={color=black},
xtick={0,0.05,0.1,0.15,0.2},
xticklabel style={font=\large, text width=0.8cm},
xticklabels={0,0.05,0.1,0.15,0.2},
xlabel={\large Occlusion level},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=-0.0182922023410576, ymax=0.345565283979908,
yticklabel style={font=\large, text width=0.8cm},
ytick style={color=black},
yticklabels={0,0,0.05,0.1,0.15,0.2,0.25,0.3},
ylabel style={align=center},
ylabel={\large Percentage of images \\ \large per occlusion level},
]
% \addplot [only marks, mark options={scale=2}, mark=*, draw=color0, fill=color0, colormap/viridis]
% table{%


\draw [fill=color0,draw=black,very thick] (-0.02,0) rectangle (0.02,0.2);

\draw [fill=color0,draw=black,very thick] (0.03,0) rectangle (0.07,0.2);
\draw [fill=color0,draw=black,very thick] (0.08,0) rectangle (0.12,0.2);
\draw [fill=color0,draw=black,very thick] (0.13,0) rectangle (0.17,0.2);
\draw [fill=color0,draw=black,very thick] (0.18,0) rectangle (0.22,0.2);
% x                      y
% 0 0.326399683952332
% 1 0.0538691021502018
% 2 0.202056527137756
% 3 0.00580210657790303
% 4 0.0077663017436862
% 5 0.0109455175697803
% 6 0.00183956371620297
% 7 0.00488027883693576
% 8 0.141013011336327
% 9 0.0102499211207032
% 10 0.0355792082846165
% 11 0.0107911732047796
% 12 0.0011962060816586
% 13 0.061921238899231
% 14 0.00236772932112217
% 15 0.0020821017678827
% 16 0.00206185271963477
% 17 0.000873397686518729
% 18 0.00366423046216369
% };
\end{axis}

\end{tikzpicture}
